SkillFence: A Systems Approach to Practically Mitigating Voice-Based Confusion Attacks

Voice assistants are deployed widely and provide useful functionality. However, recent work has shown that commercial systems like Amazon Alexa and Google Home are vulnerable to voice-based confusion attacks that exploit design issues. We propose a systems-oriented defense against this class of attacks and demonstrate its functionality for Amazon Alexa. We ensure that only the skills a user intends execute in response to voice commands. Our key insight is that we can interpret a user's intentions by analyzing their activity on counterpart systems of the web and smartphones. For example, the Lyft ride-sharing Alexa skill has an Android app and a website. Our work shows how information from counterpart apps can help reduce dis-ambiguities in the skill invocation process. We build SkilIFence, a browser extension that existing voice assistant users can install to ensure that only legitimate skills run in response to their commands. Using real user data from MTurk (N = 116) and experimental trials involving synthetic and organic speech, we show that SkillFence provides a balance between usability and security by securing 90.83% of skills that a user will need with a False acceptance rate of 19.83%.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> z_2_background.tex <==
\section{Background}
%\subsection{Alexa}
\label{sec_1_1}
%Smart voice assistants, like Amazon Alexa and Google Home, have grown to control physical devices in homes~\cite{alexa-iot}, perform financial transactions~\cite{alexa-finance} and help educate young children~\cite{alexa-forkids}. They accomplish such diverse functionality using advances in human speech interpretation and a third-party application model where developers create \emph{skills}\footnote{We use Amazon Alexa terminology.} (voice-based apps). Skills can be conveniently developed with the supports from Amazon and Google, via Alexa Skills Kit and Actions on Google. Voice assistants are popular, with approximately 60 million people in the US alone owning a smart speaker in 2020~\cite{speakersalestats}. Although these devices are useful, they present security and privacy risks.
\noindent{\textbf{Alexa Ecosystem.}} The Alexa ecosystem consists of a device placed in a user's home (e.g., smart speaker), a cloud platform implementing general voice assistant functionality, and an application endpoint implementing skill-specific functionality. The automatic speech recognizer (ASR) receives a command from the user and converts it to text. The natural language understanding (NLU) unit performs syntactic and semantic text analysis. to determines the most appropriate \appv matching the user's utterance. The \appv developer hosts a cloud endpoint that implements the functionality API. For example, if the user utters \textit{``Lyft, Get me a car''}, the ASR and NLU will eventually determine that Lyft can handle the command. Thus, the \avS cloud platform sends a message to the HTTP(s) API endpoint for Lyft. 
Skill developers provide the directory entry information, and they are in complete control of all aspects of that data. This includes the skill name, invocation phrase, suggested commands and URLs for privacy policies and account linking. 

% and looks up a directory to compute the endpoint
%  by looking up the directory

%Current voice assistants only perform superficial metadata checks. For example, they will ensure that a new skill does not completely copy the graphics and name of a popular skill and will perform basic functionality tests~\cite{alexa-functionality-testing}. Unfortunately, this type of vetting is not foolproof and does not scale well. In Section~\ref{sec:metadata-attack}, we discuss a case study where we created an attack skill that squats on the FitBit skill while replicating FitBit's account linking URL.


%still needs a bit of work -- we need to discuss. The automating enabling is still not coming across. 
\noindent{\textbf{Skill Invocation.}} \mjrev{
Amazon Alexa allows users to perform two skill operations - enabling and disabling. These operations can be executed via the skill's Amazon listing. Additionally, to promote usability Alexa automatically enables a skill when it is invoked by the user (e.g.,``Open Fitbit''). Once enabled, the skill can also be implicitly invoked (e.g., ``Ask Fitbit how I slept last night''). Lastly, a currently disabled skill cannot be invoked until it is explicitly re-enabled.}

%Users primarily interact with skills in three ways --- modal interaction, one-shot invocation, and skill suggestion~\cite{askAlexa}. Modal interactions are explicit invocations where the user first invokes a skill (e.g., ``Open Twitter'') then issues a command (e.g., ``Search for trending tweets''). One-shot invocation can implicitly interact with a skill, for example, ``What's trending on twitter.'' Skill suggestion explicitly asks the user's choice from a set of candidate skills. The one-shot invocation is only available for the skills a user has \emph{enabled} previously. Each skill belongs to one of three states: Enabled, Disabled, and Untouched. Initially, all skills belong to the Untouched state. Any skill can be \emph{enabled} through either the skill's listing on the Amazon website or when the user invokes it for the first time. Similarly, any enabled skill can also be disabled by the user. To use a disabled skill, it needs to be re-enabled via the skill's Amazon listing or by voice where the user need to explicitly say  ``Enable <skill name>'', followed by a confirmation~\cite{disableskill}. }

%\noindent{\textbf{Amazon Policing.}}
%\label{sec:amazon_policing}
%\textcolor{blue}{ Given Amazon's familiarity with the aforementioned NLU and ASR pecularities, along with its ability to accept, reject, and remove skill submissions, one might wonder why Amazon cannot solve potential security issues for its Alexa users as the central controlling entity. Unfortunately, Amazon has a distinct disadvantage in this case. Top-down solutions from Amazon incur numerous additional security and privacy issues that do not exist with a user-oriented bottom-up systems approach. For example, were Amazon to begin policing user skill libraries for malware, a number of complications occur. How often would Amazon monitor these user skill libraries? What happens if this information is misplaced? Which skills would be labeled as dangerous? And most importantly, how would the phonetic landscape of the market change once dangerous Skills are detected? A top-down approach is necessarily disincentivizing for either established developers or new developers because the central entity must prune existing skills in a nearby phonetic space or limit the phonetic properties of new skills to prevent skill squatting instances. In either case, the growth of the Alexa marketplace is hindered. 
%\paragraph{}Instead, we provide Amazon with two Alexa ecosystem recommendations, which are simple to implement and provide increased user security. These recommendations strengthen SkillFence's ability to provide user security, but they are not necessary for SkillFence to work effectively in the marketplace's current form.}

%\noindent{\textbf{Account linking.}}
%When a user activates a skill, they must link their account so that it can access sensitive information. For example, to order a cab with Lyft, the user must authorize the Lyft skill to access their Lyft account. This occurs through the \emph{account linking} process. The skill developer specifies an account linking URL in the manifest at development time. At run time, the user navigates to this link, logs-in, and authorizes the skill to the account. This process occurs through a delegated authorization mechanism like OAuth.

%\color{black}
%\subsection{Voice Confusion Attacks}
%\label{voice_confusion}
%Beyond traditional computer security vulnerabilities, recent work has shown \avP to be vulnerable to \textit{voice-based confusion attacks}~\cite{kumar,zhang,lipfuzzer}. \color{blue}These attacks exploit a combination of fundamental issues with voice assistant design: (1) lack of skill metadata vetting, (2) errors in interpreting speech, (3) user difficulty in verifying the skill being executed, and (4) tension between usability and security.



%\color{black}



%Consider a skill that allows users to interact with the Capital One bank. A malicious skill might have the name \textit{Capitol Won}. The speech recognition systems can confuse both skills, and invoke the malicious skill, instead of the true banking app, without the user knowing. To improve usability, \avP  have introduced auto-enabling features where the skill directly executes after the user speaks~\cite{alexa-no-perm-prompt} without any further involvement. Once activated, such a skill can steal private information~\cite{shezan-www2020} or perform other dangerous actions. Similar attacks attempt to mimic the voice interface of legitimate skills~\cite{zhang} or rely on semantic interpretation errors of natural language understanding~\cite{lipfuzzer}. All these attack techniques result in the same effect of getting the \avS to execute a skill that the user did not intend or expect. They define a broad class of voice-based confusion attacks on \avP targeted at end-users.





==> z_7_security_analysis.tex <==
\section{Security and Privacy Analysis}\label{security-analysis}
% reiterate assumptions for security guarantees.
Per our threat model, the attacker is a malicious skill that tries to get executed by leveraging various design flaws in the Alexa ecosystem. The user's browser, smartphone and the legitimate skill developer's websites are trusted and not compromised. An attacker could try to compromise a legitimate website to include a fake link to their attack skill. Because of \sys\xspace however, the bar for the attack is now much higher than just uploading a malicious skill to a loosely-vetted marketplace.




% adaptive:
% 0. attacker tries to compromise legit website.
% 1. attacker injects text on website that supports user-generated content to trick backlink analysis
% 2. attacker tricks user into visiting fake website so that their counterpart activity is poisoned
% 3. attacker can try to create a phonetically-close skill JUST outside the phonetic radius threshold we set. 
% 4. privacy-respect collection of web+android history: no transmit

\subsection{Adaptive Attack Analysis}
We consider an adaptive attacker with knowledge of how \sys\xspace works. Concretely, this attacker can: (1) trick the user into visiting a fake website such that the counterpart activity  is poisoned; (2) inject text on a legitimate skill developer website that supports user-generated content so that the backlink analysis is tricked; (3) create a skill whose invocation phrase is just outside the phonetic radius of the legitimate skill in an attempt to still leverage voice confusion attacks. As we discuss below, our work prevents these attacks by design. 

\noindent\textbf{Counterpart activity poisoning.} \rev{An attacker can trick the user into clicking on websites they control and link those websites to a malicious skill }. This can result in malicious skills getting enabled because \sys\xspace mistakenly interprets the malicious websites as the user's intention. \sys\xspace prevents this attack using its website history filtering technique discussed in Section~\ref{site_history_filter}. An attacker could also try to trick the user into installing an Android app they control. This is a harder task than just uploading a malicious skill to a loosely-vetted marketplace. The attacker has to create an Android app, get it past Google Play's strict vetting policies~\cite{alexavetting, hu2020case} and then trick the user into installing the application. Thus, \sys\xspace raises the bar for a voice confusion attack.

\noindent\textbf{Fake URL injection on legitimate website.} If a legitimate skill developer's website supports user-generated content (e.g., a help forum), an attack can insert a URL to their attack skill, thus tricking \sys\xspace into linking the legitimate website's identity with the fake skill. Our backlink analysis prevents this attack by excluding user-generated pages.

\noindent\textbf{Phonetic threshold attack.} The malicious skill developer can choose an invocation phrase that lies just outside the phonetic cluster of an enabled skill. This can lead to a voice-based confusion attack. In Section \ref{eval_enable_disable}, we demonstrate that the probability of incorrect invocation decreases for a higher threshold. Hence, choosing a conservative threshold makes it harder to induce a voice confusion attack.

\subsection{Privacy Analysis}
The \sys\xspace extension accesses website history and list of installed Android apps. \rev{However, it does not store any of this information, not even on the locally. It also does not transmit it to the server, and only receives the mapper table}. It just computes on this information locally using the mapper table. The only information communicated to Amazon is the set of enabled and disabled skills. The set of enabled ones can leak a small amount of information to Amazon if there are skills that user does not eventually use. Concretely, it leaks information that a website corresponding to that skill was visited. This is a small amount of information compared to existing privacy issues with systems like voice assistants~\cite{alexavetting, hu2020case, shezan-www2020} and is reasonable compared to the security advantage of preventing voice confusion attacks.




%In this work we also consider the attacker's response to our system. There are two compelling approaches an adaptive attacker could use to circumvent the intended use of \sys. Firstly, the attacker could attempt to ``poison" the phonetic skill graph by creating skills with invocations within a close phonetic distance to the user’s legitimate invocation phrases in an attempt to increase the probability of their adversarial skill being executed. Secondly, a motivated attacker could create a combination of malicious web pages and companion skills in an attempt to circumvent \sys's web history filter. 

%\paragraph{\textbf{Graph Poisoning}}
%For graph poisoning to be effective, an attacker would first have to bypass the initial web history screening. A poisoned graph does not give any advantage to the attacker, as any skill that is screened out will be disabled up front prior to the execution of any user skill. Therefore, the attacker does not gain an advantage by attempting to poison the phonetic graph.

%In the case where attackers go so far as to copy the invocation and URL data of a skill that a user genuinely uses, they are still unsuccessful unless they phish the user on the web. Our defense raises the bar for an attack. Previously, attackers had the capability to luck into a scenario where natural language ambiguity or imperfections in the voice assistant ASR were able to grant their skill execution. Now, though, the attacker must successfully phish the user across multiple web sessions in order to have the ability to launch a skill squatting attack at all. 

%\paragraph{\textbf{Web History Screen Subversion}} 
%This adaptive attacker who attempts to bypass the web history filter has two variables to manipulate: attacker-controlled malicious skills and attacker-controlled malicious websites. Thus, there are four different permutations for an attacker to adjust. The following are the possible permutations, each of which is discussed in-depth below, aside from the "one skill to one website" case, which is considered a necessary part of a voice confusion attack when our defense is in place (this case is discussed in section \ref{site_history_filter}):
%\begin{enumerate}
%    \item Many Websites to One Skill
%    \item Many Skills to One Website
%    \item Many Websites to Many Skills
%    \item One Skill to One Website
%\end{enumerate}

%\paragraph{\textbf{Many Websites to One Skill}}  One potential attack vector is through the mass insertion of pop-up spam. Our web history filter is designed to remove these spam entries by defining the time window for any url as the longest time period that elapses between any two url accesses of one site. By using this method, the filter cannot be “gamed” into passing spam pages that cause many pop-ups in a row in hopes of bypassing the time-window filter. Our web history screen ensures that a scattershot web attack from an attacker, wherein the attacker launches many spam websites linked to one skill with the hope that one will catch the user’s attention, would not succeed because spam visits are filtered out. Further, the attacker does not gain any additional advantage by controlling multiple spam sites since a skill is not authenticated by more than one website, and as mentioned previously, each skill-linked site must be visited by the \sys \xspace user in a genuine manner for the site to be considered as a legitimate link. 

%\paragraph{\textbf{Many Skills to One Website}}  If an attacker links many skills to a single site and that same site links back to the aforementioned skills, it is more likely to benefit them in bypassing our screen. If an attacker could convince a user to visit an attacker-controlled site from a skill page on the Alexa Marketplace and place similarly convincing skill pages elsewhere on the Amazon Skill Marketplace that link to the same attacker-controlled site, the attacker would succeed in bypassing our history screen, assuming the visits are far enough apart. If the user downloads any one of the skills in this case, it will automatically be enabled. An example of this is the case where two skills are produced by the attacker. 

%Let “skill one” be introduced to the user on its marketplace page as accomplishing a different task than it does in reality, and also let this skill have its true invocation phrase hidden, along with its stated permissions. Assume the user downloads this skill. Then, let “skill two” be another skill authored by the same attacker, and let “skill two” have some compelling but benign reason for causing a user click and subsequent routing to the attacker-controlled site, which is also benign in nature but interesting enough for a user to click around on for a bit. If the attacker site has back-links to both “skill one” and “skill two”, the attacker has successfully bypassed our web history screen. This adaptive attack is addressed by removing URL page visits that occur as a result of clicks on skill pages from the \sys \xspace user's web history. We employ this measure in the web history filtering process to avoid the potential of such a threat.

%\paragraph{\textbf{Many Skills to Many Websites}} Even if the attackers control a large number of sites, the utility of doing so from the attacker's perspective is limited by the number of skills a user has. Linking many sites to many skills does not give the attacker an advantage, unless the skills backlinked to their sites are already downloaded by the user. The previously-stated filtering processes still apply, and since an attacker does not gain a strategic advantage from a many to one mapping from skills to websites or vice versa, they do not gain an advantage in a many-to-many attack either. 

\color{black}

==> z_9_discussion_and_limitations.tex <==
\section{Discussion and Limitations}

\noindent{\textbf{Reliance on Chrome and Android.}}
Currently, \sys\xspace requires users to have a desktop Chrome browser, and if the user wishes to use counterpart applications for skill prediction, the apps must originate from the Android ecosystem. Future versions of \sys\xspace can easily be ported to other browsers. The current implementation likely sees a more fragmented picture of the user's web history than it would were it available on each of the major browsers.


%Future iterations of \sys\xspace can be ported to Firefox with minimal changes, as our extensions implementation was written in vanilla JS. With the release of Mac OS X 11 Big Sur, Chrome extensions are automatically convertible for use in the Safari browser. The current \sys \xspace implementation likely sees a more fragmented picture of the user's web history than it would were it available on each of the three browsers mentioned above.

\noindent{\textbf{Lack of Secure Identity for All Skills.}} The number of skills we can securely link to their website counterparts and automatically enable is limited by the number of skills with backlinks present. If a non-malicious skill lacks a URL backlink from the developer website to the skill URL, our system is unable to derive a secure identity. As we discuss in our design recommendations (previous section), a small change on the skill developers' websites will alleviate this issue. 



% \noindent{\textbf{User-Generated Site Content.}} Our skill matching process links a skill's Amazon URL to a website if that skill URL appears on the website. Attackers can trick this process if a website allows user-generated content (e.g., a comment box or forum post). Our prototype uses heuristics to filter out this type of content. Longer term, if the stakeholders adopt our design recommendations, this problem becomes a non-issue because the skill developer and voice assistant vendor co-operate to provide the secure identity.

%does not currently filter this type of content during matching. However, we observe that future prototypes can filter out known parts of the HTML tree that contain user-generated content. 

%\paragraph{\textbf{Long-Term Considerations}}
% We recommend that voice assistant manufacturers and skill developers follow the skill \emph{metadata recommendations} introduced in Section \ref{our_recommendations}. The metadata changes suggested there remove the need for the website link crawling component of our system and provide an effective long-term strategy to link secure identity on the web to Alexa skills. 
 
\noindent{\textbf{Improvements in ASR.}} Improvements in ASR and NLU are complementary to our solution, but they alone are not sufficient to solve the voice confusion attack problem. Natural language ambiguity instances are possible as long as Amazon allows similar or identical-sounding invocations to be used by multiple developers. A policing effort by Amazon to remove such skills would hinder the Alexa Marketplace's growth while disenfranchising either new developers, old ones, or both. Because of this, our solution's contribution is not diminished in the case where Alexa's ASR or NLU technology is improved.

% we already discuss this in design reco.
%\paragraph{ \textbf{Security and Usability Trade-off}}
%The ideal \sys \xspace design would involve disabling all skills except the authorized ones that we identify based on the user's activity with counterpart apps. Unfortunately, the Alexa skill API only offers a method that disables a single skill at a time. Given that users only need a small fraction of skills compared to the market size, the disable operation is very expensive due to network round trips. Thus, our optimization is to determine a small set of skills that are within a phonetic radius around an authorized skill and only disable them. Should the user wish to be more conservative and incur a larger initial configuration time, \sys \xspace can expand the phonetic ring within which skills are disabled. The larger the phonetic ring, the safer the user skill is against potential voice confusion attacks.


%We recommend that voice assistant manufacturers provide an API that can efficiently disable a large list of skills with a single network call, as recommended in Section \ref{our_recommendations}'s \emph{Enable/Disable Recommendations}. This addition, when used in conjunction with \sys \xspace,  would allow for the complete elimination of voice confusion and total assurance of correct execution for the user.

\color{black}

==> z_implementation_and_evaluation.tex <==
\section{Evaluation}\label{sec:evaluation}

We perform an end-to-end evaluation of \sys  and it's core components. We summarize our evaluation findings, then discuss the experimental setup and finally provide experimental details. We also discuss how \sys's design protects against an adaptive attacker with the knowledge of how \sys works.

\subsection{Evaluation Overview}
 
 Our evaluation answers the following questions:
\begin{itemize}
     
     %We test \sys's ability to securely map user's intentions to skills by performing a trace-based evaluation on the data collected from a user study. On average, \sys  is able to securely map \predVal of the skills of a user. For the ideal scenario where all developer websites provide backlinks to their skill's Amazon listing, \sys  is able to securely map \predIdealVal of a user's skills.

    %\mnotes{We should switch q2 and q3's order once we are done editing the content of each}
    %\item[\textbf{Q2.}] \textbf{How effective is \sys  in preventing skill squatting attacks against identified skills?  End-to-End Evaluation} \\
    %{
     %We perform trace-based runtime voice experiments in the live Alexa environment.
     %We demonstrate that \sys  provides end-to-end protection against skill squatting. Across all users in the user study, we find that \sys  is able to reduce incorrect skill invocations from  9 to 6\ah{Change this if we cannot add backlinks}. For the ideal scenario where all developer websites provide backlinks to their skill's Amazon listing, \sys  can reduce incorrect skill invocations to 2.
    %}
    
    \item[\textbf{Q1.}] \textbf{\textit{What are the characteristics of Alexa Enable/Disable API in controlling which skills get executed?}}
    %How effective is \sys  in preventing attacks against the skills vulnerable to voice confusion?
    %We perform a set of runtime experiments in a live Alexa environment. 
    
    We test \sys's Enable/Disable module against vulnerable skills registered on the Amazon Marketplace. These vulnerable skills include ones that share invocation phrases or have similar sounding invocations.
    %Through a number of trials on skill sets of various sizes with identical invocations, we show that incorrect or failed routing instances occur at unacceptable rates.
    %We demonstrate that \sys is able to bring down the rate of incorrect invocations from 27\% to 0\% for skills with similar sounding invocations.
    %\ah{Matt, add a similar one line for identical invoke experiments}
    %For this set of experiments, we select many newly-identified at risk skills, along with the set of skills shown to be potential voice confusion targets by past work. We select these skills so that \sys 's efficacy in defending known vulnerabilities is demonstrated. Furthermore, the skills collected in the user study are primarily known to have few, if any, similar skills and thus are not prone to skill squatting. Our deliberately selected set of skills provides a better evaluation of \sys’s ability against possible squatting attacks. We show that \sys  prevents skill squatting and also reduces instances of arbitrary routing for identified skills. \kj{Do we have any metrics that we can add here? Something looks missing here}
    
    \item[\textbf{Q2.}] \textbf{\textit{What performance overhead would a user experience while using \sys?}}
    \mjrev{
    The user-facing \sys extension performs counterpart activity collection, Mapper table indexing and enabling/disabling of the securely predicted skills. While counterpart activity collection is a batched operation and mapper-table indexing happens locally, enabling/disabling is the most time-consuming step. The initial setup time depends on the phonetic distance threshold and can vary between 17 minutes to 3 days. A security favouring distance threshold requires a longer setup time. Subsequent \sys operations encounter fewer enabled skills at a time, leading to a much quicker response time of less than a minute.
    }
    \item[\textbf{Q3.}] \textbf{\textit{How effective is \sys in preventing voice confusion attacks? How does \sys balance the security-usability trade-off?}}
    
     %We perform a trace-based evaluation. %--determining user's choice among ambiguous invocations
     %--end to end attack reduction
     %--usability-security trade-off - FAR, FRR
     %--setup time
     \mjrev{We perform a trace-based evaluation with real user data from our data collection effort. For a distance threshold of 500, \sys is able to perform at a False Rejection Rate of 9.17\%, a False Acceptance Rate of 19.83\% and an Equal Error Rate of 16.5\%.}
     %We perform a trace-based evaluation with real user data from our data collection. \sys's effectiveness comprises two pieces: (a) how many of a user's skills can it securely predict from counterpart data; (b) once a set of skills are predicted and enabled, can the system mitigate voice confusion attacks. For $N=$ \numUsers users, \sys can predict \predIdealVal of the skills on average. Furthermore, once the predicted skills are enabled and the phonetic neighbors are disabled, \sys is able to reduce incorrect skill invocations by $77\%$. 
    
    \item[\textbf{Q4.}] \textbf{\textit{How does \sys protect against an adaptive adversary? What are the privacy implications of using \sys?}}\\
    The different components of \sys are designed to address an adaptive attacker and make it more challenging to launch a successful attack. \sys does not maintain any state or store any user information, even locally, minimizing any privacy concerns.
    
    \color{black}
    %The user-facing \sys extension performs counterpart activity collection, indexing into the Mapper table and enabling/disabling of the securely predicted skills. Counterpart activity collection occurs during periods of browser inactivity. Thus, users do not directly experience overhead. Indexing into the Mapper table occurs locally and has minimal overhead. The most  Enabling/Disabling skills takes on average $4$ minutes (based on our trace-based evaluation of real user data), and this is the most time-consuming operation. We observe that this happens in the background --- the user is not involved in the process. Furthermore, this is a one-time setup cost. Subsequent \sys operation will encounter fewer enabled skills at a time, leading to a quicker response time. Finally, this overhead is an artifact of our implementation that works with an unmodified Alexa system. Our design recommendations (Section~\ref{our_recommendations}), if adopted by voice assistant manufacturers, will reduce this overhead to negligible values. 
    
\end{itemize}

%  

\subsection{Q1. Enable/Disable Module Evaluation}\label{eval_enable_disable}
\sys relies on the Alexa enable/disable API to ensure that securely predicted skills execute despite the presence of phonetically-close skills. In the prior section, we demonstrate that when the predicted skills are enabled and when the phonetic-neighbors are disabled, Alexa executes the enabled skills only.  In this section, we perform large-scale voice experiments to characterize this behavior and show that the act of enabling a skill out of a set of phonetically-close skills while disabling the rest always biases Alexa to execute the enabled one. 

%As discussed previously, in an ideal world
Ideally, there would be a single API that would let us disable a large set of skills (because users only interact with a small subset of skills compared to the universe of skills). However, Alexa does not offer this API. To strike a reasonable balance between performance and security, \sys instead computes the set of skills that lie at a certain phonetic distance away from the enabled skill and only disables those. Our experiments use a threshold of 400. In this section, we discuss how we empirically tuned this number. 

%The previous section demonstrates \sys's ability to protect a user's critical skills. However, most of the evaluated skills do not have other phonetically similar skills that may pose invocation ambiguity. Hence, we evaluate \sys 's ability to prevent skill squatting for the most vulnerable skills on the Alexa market. Part of our findings show that a phonetic distance threshold of 400 is able to prevent every skill squatting instance from our experiments. 

%We also demonstrate that a distance threshold of more than 400 is able to prevent skill squatting instances. 

\subsubsection{Experimental Setup} The high-level approach is to repeatedly invoke sets of phonetically-close skills while manipulating which one is enabled/disabled and then observing the results. We created the following two datasets:
\noindent\textbf{Dataset of skills with identical invocation phrases.}\label{identical_eval_skills} We create $8$ disjoint sets of skills where each set contains members with identical invocation phrases. The complete list of skills can be found in Appendix Sec. \ref{appendix}. Note that each skill is randomly taken from the Alexa marketplace (any repetitions in skill names and invocation phrases occur naturally). We have a total of $28$ unique skills. We constructed these sets to test \sys's Enable/Disable module against skills that share invocations with different number of other skills.
    
    
    %retrieve $8$ disjoint sets of skills, where each set only contains members with identical invocations. We randomly selected $2$ sets for each identical invocation set of size $2$ through size $5$. Thus, we have $8$ sets and a total of $28$ unique skills in this set of trials. 
    
    
\noindent\textbf{Dataset of skills with similar sounding invocations.} We select the largest set of skills with unique invocations which satisfies the property - for each skill, the set also contains at-least two other skills whose invocation phrases are at a phonetic distance of less than 500. This set of 53 skills represents a phonetically dense cluster of skills. We select these skills from the whole Alexa market rather than just the set of critical skills to find the skills that are most vulnerable to voice confusion attacks. 

For each dataset, we perform a runtime evaluation by invoking each skill on a test Amazon Alexa account. \mjrev{We feed synthesized voice using the Alexa Voice Service to directly interact with the Alexa backend. This audio is of the form: "Alexa, open <skill invocation phrase>". We terminate the interaction with the Alexa backend once the skill invocation occurs or if Alexa cannot process the request.} We classify the result of each invocation as: ``correct skill'', ``incorrect skill,'' or ``no routing.'' The last category occurs when Alexa fails to run any skill. 

\mjrev{For each experiment, we create invocation audio for using Google TTS and also use human speech reconstructed from the LibriSpeech dataset~\cite{libri}. LibriSpeech consists of transcripts for around 1000 hours of spoken English from $2484$ speakers. To construct an invocation audio from this corpus, we first search for any continuous utterance of the invocation phrase. If nothing is found, we break the invocation phrase into smaller components and stitch together the respective audio clips to create a full phrase. We ensure that the components were derived from the same speaker. Since some skill invocation phrases contain non-English words (e.g., Amex), we were not able to generate organic invocation audio for all skills in the dataset. To avoid any speaker-specific errors, we perform each trial with audio samples collected from three different speakers. Then, we take the majority result from the three outcomes.}

\begin{table}[]
\centering
\caption{Invocation Experiment - Skills with identical invocation phrases: Invocation Outcomes}
\begin{tabular}{p{0.2\columnwidth} x{0.12\columnwidth} x{0.36\columnwidth}}
\toprule
%Metric & All Enabled & Target Enabled, Others Disabled & All Disabled \\ \hline
%Correct Invocation & 2 & 23 & -- \\
%Incorrect Invocation & 4 & 0 & -- \\
%No Invocation & 2 & 5 & 8\\
Metric & Default State & Target Enabled, Others Disabled \\ \hline
Correct Invocation & 2 & 23 \\
Incorrect Invocation & 5 & 0 \\
No Invocation & 1 & 5\\
\bottomrule
\end{tabular}%
\label{identical_invocation_experiments}
\end{table}


\begin{table}[t]
\caption{Invocation Experiment - Skills with similar sounding invocations: Invocation Outcomes. Note: the number of trials varies between TTS and Audio Recording as not
all of the invocation phrases are in the LibriSpeech dataset.}
\begin{tabular}{p{0.2\columnwidth} x{0.13\columnwidth} x{0.35\columnwidth}}
\toprule
 &\multicolumn{2}{c}{\textbf{Text-to-Speech Experiment}}\\
    \cmidrule{2-3}
 %\quad\quad Metric & Both Enabled & Target Enabled, Adversary Disabled & Both Disabled \\
 %\midrule
%Correct Invocation     & 87 & 96 & 62 \\ 
%Incorrect Invocation & 5  & 0   & 30  \\
%No Invocation          & 12 & 10  & 14 \\
\quad\quad Metric & Default State & Target Enabled, Adversary Disabled \\
 \midrule
Correct Invocation     & 62 & 96 \\ 
Incorrect Invocation & 30  & 0  \\
No Invocation          & 14 & 10 \\
\toprule
 &\multicolumn{2}{c}{ \textbf{Audio Recording Experiment}}\\
 \midrule
%Correct Invocation     & 40 & 46 & 25 \\ 
%Incorrect Invocation        & 4  & 0  & 13  \\
%No Invocation          & 4  & 2  & 10 \\
Correct Invocation     & 25 & 46 \\ 
Incorrect Invocation        & 13  & 0 \\
No Invocation          & 10  & 2 \\
\bottomrule
\end{tabular}\\
% \multicolumn{4}{l}{\makecell{The number of trials varies between TTS and Audio Recording as  \\ not
% all of the invocation phrases are in\\ the LibriSpeech dataset}}
%\multirowcell{6}{The number of trials varies between TTS and Audio Recording as  \\ not
%all of the invocation phrases could be found in\\ the LibriSpeech dataset.}
\label{tab:exp_table}
\end{table}



\subsubsection{Results for Identical Invocation Phrase Dataset}

\mjrev{ADD ORGANIC INVOCATION EXPERIMENTS FOR IDENTICAL INVOCATION}
We use the Google TTS API to generate audio for invocation phrases, and run the following sequence of experiments.


%For this set of skills, we use GTTS and AVS to automate interaction with our test Alexa account. The purpose of surveying sets with identical skill invocations and various sizes is to see how Alexa's ASR handles various levels of ambiguity. To this end, we run the following trials for each set: 
\begin{enumerate}
    
    %\item Enable all members of the set, randomly pick one of them as the user's intended invocation and then play audio.
    \item Baseline: With all skills in default state, play audio for invocation phrase. The intended target is the most popular skill (with most reviews) in the set.
    \item \sys: For each member of the set, enable that member, disable the rest of the set's members, and play audio. The intended target is the enabled skill.
    %\item For N=2 to N=set size, enable N skills and execute invocation.
    
    
\end{enumerate}

In this experiment, we run $36$ trials in total. Table~\ref{identical_invocation_experiments} contains the results. The first column contains results for the first condition above. Because the simulated user's intended invocation is sampled only once and as we have $8$ sets of skills in the dataset, we have a total of $8$ outcomes. We invoke the most popular skill (with most reviews) in the set because popularity is a factor in deciding skill invocation~\cite{alexa-no-perm-prompt}. We observe that in $2$ cases, the user's intended skill is executed (`correct invocation'), in $5$ cases, the unintended skill is invoked and in $1$ cases, invocation fails. We conclude that in the presence of identically named skills, confusion does occur. 

The second column tests the second condition. Correct invocation of the user's intended skill occurs $23$ times when the intended skill is enabled and unintended ones are disabled ($5$ result in invocation failure). This trial confirms our observed behavior of the enable/disable API --- when the intended skill is enabled and phonetically close skills are disabled, only the intended skill executes in response to an ambiguous invocation phrase. 

%For each of the $8$ sets surveyed, we disable each member and execute the set's shared invocation phrase, as depicted in configuration $1$. This is done to confirm the disable action's functionality when operating on sets of skills with shared invocations. Then in configuration $2$, we iterate over each set's members and enabled a single member while disabling the rest of the set's members. This procedure is run once for each unique skill in each unique set, for a total of $28$ trials. This process emulates \sys  and demonstrates how our system handles ambiguity in practice. 

%After we have emulated our defense, we next enable every member of the set at hand and randomly select one member as the desired skill to invoke. This experiment corresponds to configuration $3$ and is run for $8$ trials (one trial for each unique set). The expected value of successes over these trials is $\sim 2.57$, assuming Alexa behaves in a uniformly random manner and each trial is independent. 

%we select one permutation ordering for each set and sequentially enable one additional member per %experiments until we have enabled all members of the set. 

%This step corresponds to configuration $3$ and is run for $20$ trials ($48$ total trials - $28$ defense-emulating trials). This procedure is executed to show the problems associated with execution accuracy that occur in the face of ambiguity in practice. Note that we do not attempt every permutation ordering because the scale quickly becomes unmanageable, and this demonstration is intended to show the existence of the ambiguity problem as opposed to exhaustively demonstrating its existence in every permutation.
%Throughout these trials, we found that sets with one or more members sharing an invocation are more likely to experience routing failures ($8/28$ instances) or incorrect routings ($23/28$ instances) when compared with the occurrences in our other experiments. Additionally, $4$ of the $5$ correct routings that occurred happened when only one skill was enabled and the rest in the set at hand were disabled. Thus, its likely that having more than one identical skill invocation enabled does increase Alexa's error rate in interpreting the user's intention. Note that $36$ trials in total were run, but that the $8$ trials where every skill is disabled are not accounted for in the aforementioned figures; these trials were done to confirm that the disable action functions similarly when multiple identical invocations are being disabled. Note that we do not attempt every permutation for this set of trials and instead opt to use one permutation for each set. Table \ref{identical_invocation_experiments} contains the comprehensive results for the trials described here.


\subsubsection{Results for Similar Invocation Phrase Dataset}
 \mjrev{In this experiment,} we conducted the invocation trials by selecting pairs of skills $(A,B)$, such that skill $B$ is the phonetically closest one to skill $A$. By design, there are $106$ such pairs when we use Google TTS and $48$ such pairs when we use reconstructed human audio. For each pair, we test the invocation of skill $A$ in three configurations:
\begin{enumerate}
    %\item Baseline: Both Enabled (skill $A$ enabled, skill $B$ enabled)
    \item Baseline: Default State (skill $A$ disabled, skill $B$ disabled)
    \item \sys: Target Enabled, Adversary Disabled (skill $A$ enabled, skill $B$ disabled)
    
\end{enumerate} 
Configuration (1) is the control condition that tests how Alexa responds to confusing voice commands currently. Configuration (2) simulates the case where \sys predicts that skill $A$ is the user's intention.  

Table~\ref{tab:exp_table} shows the skill invocation results for both GTTS and organic audio. Configuration (1) incurs $28\%$ and $27\%$ incorrect invocations respectively for the two modes of audio. For configuration (2), the number of incorrect invocations is zero. Thus, we conclude that the behavior of Alexa supports our hypothesis: when a skill is enabled and its phonetic neighbors are disabled, the voice assistant will automatically execute the enabled one. 

%However, for both the sets, Configuration (2) has no incorrect invocations. This demonstrates that \sys  prevents skill squatting even for highly vulnerable skills.  
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\columnwidth]{images/incorrect_routing_dist.pdf}
    \caption{Invocation Experiment - Skills with similar sounding invocations: Phonetic Distance between all skill pairs that resulted in incorrect routing. There are no incorrect pairs beyond a distance of 400.}
    \label{fig:incorrect_routing_dist}
\end{figure}

\subsubsection{Enable/Disable Threshold Tuning}
\label{sec:tuning}
Among the trials that led to incorrect invocations, Figure~\ref{fig:incorrect_routing_dist} shows the phonetic distance between the invocation of the desired skill and the incorrect skill that was actually invoked. Incorrect invocation occurrences were more frequent between skills whose phonetic distance was smaller. Also, no incorrect invocation occurred between skills with phonetic distance more than 400. Therefore, for the current set of registered skills on Alexa, \sys, when configured with a threshold greater than 400 will be able to prevent voice-confusion attacks between any skill pair (assuming the target skill has been mapped).



%\mnotes{the note below table 2 collided with figure 8 and part of it was obscured, so I moved it into the caption of table 2 for now.}

%\begin{table}[]
%\centering
%\caption{Identical Skill Invocation Table. 28 trials where one or more skills were enabled were conducted. 8 %trials were conducted where all skills in the component were disabled. }
%\resizebox{\columnwidth}{!}{%
%\begin{tabular}{ll|l|l|l|l|l}
%\hline
%\multicolumn{7}{c}{Identical Invocation Trials} \\ \hline
% & & Correct Routing & Ambiguous Execution & Inside Routing & Outside Routing & No Routing \\ \hline
%\multirow{Component Size} & 2 & 0 & 0 & 1 & 0 & 5 \\ %\cline{2-7} 
% & 3 & 0 & 0 & 1 & 0 & 7 \\ %\cline{2-7} 
% & 4 & 3 & 0 & 8 & 1 & 1 \\ %\cline{2-7} 
% & 5 & 2 & 8 & 10 & 0 & 2 \\ \hline
%Totals &  & 5/28 & 8/28 & 20/28 & 1/36 & 15/36 \\ \hline
%\end{tabular}%
%}
%\label{identical_invocation_experiments}
%\end{table}


\subsection{Q2. Performance Overhead}

We discuss the time it takes for \sys to complete the skill enabling/disabling process. This phase is the longest operation. Concretely, we block our extension's operation for two seconds after each new skill page is loaded to avoid Amazon's robot detection measures that automatically log the user out. Thus, it takes $2.5$ seconds on average to enable a single skill and $3.08$ seconds to disable a skill. \mjrev{In Section 5.4, we estimate the average initial setup time for a user using our user study. Figure \ref{fig:setup_time} shows how the initial setup time varies for different values of distance threshold.} We observe that this process occurs in the background without user interaction. 
%\kj{should be 17 mins if we include 2 second page delay to avoid robo-detection}
This operation can be sped up using parallelization at the risk of being detected as a robot clicker. The optimal solution to this problem would avoid iteration altogether by using enable and disable functions that allow multiple skills to be selected simultaneously. Should this ability be added, the usability cost for a user's initial defense setup would be greatly reduced. Once the setup is completed, subsequent updates to either the mapper table or the user data only trigger enable/disable of a small number of skills which can be completed in around 2-5 minutes. %We further explain the positive benefits of adding this functionality to the  Enable and Disable APIs in our recommendations section (section \ref{our_recommendations}).

%On average, a single page click takes $0.54$ seconds to execute. For enabling, this incurs a $2.54$ second time cost per skill. For disabling, this incurs a $3.08$ second time cost per skill. Given that the average user in our human study had $30$ enabled skills and $50$ disabled skills, the average initial setup cost for \sys is roughly $\sim 4$ minutes. Additional tabs can be spawned for parallelizing clicks to speed up the enable and disable processes, at the risk of detection by a robot checker. 

\subsection{Q3. End-to-End \sys Performance}
\label{end_to_end_effectiveness}


\subsubsection{Experimental Setup}

Our experimental setup consists of two steps. First, we initialize the backend component of \sys; we crawl the Alexa skill market to collect the metadata (skill name, developer, invocation name, URLs, etc.) of each skill and populate the Mapper Table. Second, we perform a data collection campaign to study the performance of \sys over real-world user data.

We choose to focus our analysis on a subset of the Amazon Alexa skill Marketplace: the \acLinkingSkills skills with account linking, which represent the sensitive skills on the Alexa market according to a recent analysis by Shezan et al.~\cite{shezan-www2020}. Account linking skills are likely to be the targets of attack because of their access to the user's account data. We designate skills that have account linking as critical. Note that \sys's design, implementation, and evaluation can be readily applied for the full set of skills without changes to the Alexa Marketplace or how skills operate on the Alexa platform. 

%%%Kassem: Is the below needed?
% However, by focusing on a smaller set of sensitive skills, we reduce the experimental artifacts resulting from the user study that involves extracting user data only once. Any additions or removal of skills on the Amazon Marketplace, as well as updates to skill metadata during the lifetime of the user study will lead to inconsistent results. Once deployed, periodic functioning of \sys  will handle these issues.

 \begin{figure}[t]
    \centering
    \includegraphics[width=0.5\columnwidth]{images/distance_market_cummulative.pdf}
    %\label{fig:dislit}
    \caption{CDF of phonetic distance between invocations of all possible Skill pairs. More than 95\% skill pairs have phonetic distance > 400. All skill squatting examples cited in previous work lie within a phonetic distance of 250.}
    \label{fig:dislit}
\end{figure}

\noindent\textbf{Mapper Table}\label{sec:mapper-table}
We generate the Mapper Table for the \acLinkingSkills Amazon Alexa skills with account linking. This process includes running the backlinking analysis to extract the secure links of the skills and constructing the phonetic graph. 

\noindent\textit{Backlinking:}
The majority (2496 out of \acLinkingSkills) of skills contain at least one valid unique domain in their provided metadata. Skills that share domains generally belong to the same developer. A skill-domain pair is part of the Mapper Table only if a website associated with the domain lists a link to the skill's Amazon homepage. To search for backlinks, we follow two approaches -- Google Crawling and Link Backtracking Services. For Google Crawling, we constructed queries like "site:$<$domain name$>$ Amazon Alexa Skill" and searched through the top 100 results. We also used additional text phrases such as `Alexa Skill,' and `Amazon Skill,' to exhaustively search for all Alexa skill references. These queries provided at least one search result for 2023 skills. Among these, we found backlinks for 404 skills. For building a more exhaustive backlink profile, we utilize a Search Engine Optimization (SEO) service, \textit{Ahref}\footnote{\url{https://ahrefs.com/backlink-checker}}, which provides a tool for retrieving all backlink references for a given URL. Overall, employing both approaches, we were able to find the backlinks for 474 skills. This number is likely to increase as websites start adding references to their skill's homepage like they currently do for their Android and iOS apps. 

% We found that 1452 out of \acLinkingSkills skills have at least one backlink. 
\noindent\textit{Phonetic Graph:}
Then, we constructed the skill phonetic graph consisting of \totalSkills skills. Figure~\ref{fig:dislit} shows a CDF of weight values in the Phonetic Graph, i.e., the phonetic distance between all pairs among \totalSkills skills. We observe that only 5\% of the weights lie below the value of 400. Hence, pruning all weights more than 400 leads to a sparse Phonetic graph and considerably reduces the number of skills to be disabled. On the other hand, we observe no incorrect invocations for skills pairs with distance greater than or equal to 500. Figure~\ref{fig:dislit} also shows that all skill squatting invocation pairs introduced by previous work have phonetic distances less than 500~\cite{zhang,kumar}. Hence, there exists a trade-off between restricting the number of skills to be disabled and identifying potential skill squatting pairs.


\noindent\textbf{Data Collection:}
We perform a data collection campaign to collect installed mobile apps, skill-relevant browsing history, and preferred Alexa skills from a set of individuals through Amazon Mechanical Turk (MTurk). This data allows us to perform trace-based evaluation of \sys's extension component. %Initially, we planned to collect data from iOS and Android users, but iOS lacks the ability to extract the list of installed apps programmatically. 
We focused the data collection on individuals who own Alexa devices and Android smartphones. We obtained IRB approval for the data collection procedure from our institution. 

\noindent\textit{Data Collection Design}
We designed a Qualtrics survey hosted on MTurk to guide individuals through the data collection procedure. The survey consists of five sections: eligibility, Chrome extension installation, data collection, data validation, and clean-up. After completing a consent form that verifies age, Alexa ownership, and records the MTurk ID, the participants install a Chrome extension and log into their Amazon and Google accounts. The users enter their MTurk IDs again in the extension as a verification check. 

The data collection procedure involved two components: (1) extracting user data consisting of enabled skills, browsing history, and installed Android applications; and (2) validating this information through a survey form. We created a Chrome extension to automate data extraction. This extension scrapes the enabled Alexa Skills from a user's  ``Your Skills" page on \textit{alexa.amazon.com}. It also scrapes the user's ``My Android apps'' page on \emph{play.google.com/apps} to obtain the list of installed Android apps. In the browsing history, the extension only searches for URLs whose root domains are part of the Mapper Table.

There are two potential problems with the extracted data. First, the user could have cleared their browsing history. Second, a user might have enabled a skill with which they do not interact. This first issue applies only for the data collection and does not affect \sys  as it runs continuously at the user's side. However, after the extension is finished collecting the data, the survey populates a list of domains (domains that are mapped with any of the user's enabled skills) and asks the user to select all domains that they would have visited.

For the second issue, we define {\em used skills} as the enabled skills the user frequently interacts with. To address potential over-represented skills in the data collected (those enabled but not used), we ask the user to validate the extracted data. The survey also populates all the extracted enabled skills, along with each skill's title and a screenshot of the skill's Amazon homepage, and asks the user to select all skills that they interact with. For both the questions, additional random records (20\% of the total records) are added to the populated list. This acts as an attention check for the user. Any user that selects the additional records is removed from the analysis. When the survey detects that it has received the list of apps and skills using the participant's MTurk ID, it guides them to uninstall the app and the extension.

\noindent\textit{Data Collection Procedure}
We recruited \numUsers individuals through Amazon's MTurk who satisfy the eligibility criteria of age and device ownership. We did not enforce any additional qualifications because the survey has built-in safeguards that ensure the participants correctly installed and executed the app and the extension.  We paid each participant $\$3$ for completing the survey; 95\% of the respondents finished the survey within 9.7 minutes. The rest of the participants faced some technical issues while installing the extension, and we helped them through the process using email. This communication did not affect the anonymity of the data. Finally, we collect the lists of installed Android apps, visited web domains, and preferred skills from these \numUsers individuals. 

We conduct a preliminary check to test whether all the skills from the data collection were included in the Mapper Table. We found that 39 skills out of 69 skills were not present as their backlinks were not listed on the websites. We manually added entries for these skills to the mapping table. We performed the backlinking through interacting with the official support accounts over email and social media of these skills and disassembling their official mobile apps. 

\mjrev{
\noindent\textbf{Characterizing Errors:} 
We evaluate \sys in terms of two types of errors - (1) False Rejection Rate (FRR), and (2) False Acceptance Rate (FAR). FRR measures the probability of a used skill being rejected. For \sys, this corresponds to the probability of a used skill being disabled. FAR measures the probability where a malicious skill is missed by \sys and is not disabled. In Section x, we show that a pair of skills with a phonetic distance of more than 400 do not lead to ambiguous invocation. Using this empirical measure, we consider unused skills, with a distance of less than 400 from any used skill, to be malicious. 
}





%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\columnwidth]{images/ndss-2021/back_link_threshold.pdf}
%    \caption{\textbf{Matched skills vs Rank threshold:} Demonstrates the number of skills with backlinks for different values of rank threshold}
%    \label{fig:back_link_threshold}
%\end{figure}

%\begin{figure*}[!t]
% \centerline{
%\subfloat[\textbf{User Study Critical Application Correlation:} %Demonstrates the ratio of enabled critical skills over the total number of critical skills present.]
%{\includegraphics[width=3.25in]{ccs-2021/images/recovered_vapps_ratio_54.pdf}%
%\label{fig:crit_app_correlation}}
%\hfill
%\subfloat[\textbf{User Study Critical Application Correlation(Ideal case):} Demonstrates the ratio of enabled critical skills over the total number of critical skills present for the ideal case when all skills pass the backlink filter]
%{\includegraphics[width=3.25in]{ccs-2021/images/recovered_vapps_ratio_ideal_54.pdf}%
%\label{fig:crit_app_correlation_ideal}}
%}
%\caption{
% User study - 
% Ratio  of  each user's critical  skills intersecting  with  the  suggested  set  over  the  total  critical  skills for different phonetic distance thresholds}
%App-Skill Correlation user study results analyzing the critical skills chosen by \sys  and all critical skills
% User Study Graphs
%}
%\label{fig:user_study}
%\end{figure*}  

%\ifnum\flagShowFigTable=1
%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.5\columnwidth]{images/recovered_vapps_ratio_ideal_57.pdf}
%    \caption{\textbf{User Study Critical Skill Prediction Rate: } demonstrates the ratio of critical skills predicted by \sys  over the total number of preferred critical skills.}
%    \label{fig:crit_app_correlation}
%\end{figure}
%\fi

\mjrev{
\subsubsection{Results}
Using the data from our collection effort, we perform a trace-based evaluation of \sys to study it's effectiveness in ensuring invocation correctness for these skills despite the presence of voice confusion attacks. We also evaluate \sys's performance in terms of FAR, FRR and configuration time.}

\mjrev{
\noindent\textbf{Skill Enable Accuracy.} 
For each user, we generate a list of critical mapped skills by running the extension module on the collected counterpart data. Recall that the set of critical skills are ones that are likely to be squatted upon~\cite{shezan-www2020}. This involves extracting certificates from the visited websites and installed Android apps and then indexing the Mapper table. This produces a set of suggested skills. We then look at the phonetic neighbourhood (distance threshold less than 400) of each of the user's used skills (reported in the data collection). As this phonetic neighbourhood represents skills that can cause ambiguous invocations, we use set of suggested skills to enforce the user's preference. Hence, \sys's effectiveness is represented by the percentage of used skills that can be identified among their neighbourhoods.
 Across all users ($N=$ \numUsersTotal), for a distance threshold of 500, \sys is able to correctly enable the user's preference for \coverage of critical skills that a user is likely going to interact with. Figure~\ref{fig:crit_app_correlation} shows the distribution of the enable accuracy across users. }
%A total of $69$ unique skills existed across all users (some of these were common across users making for a total of \totalUserSkills installations). Out of the $69$, our Mapper table had entries for $21$. This represents the number of skill developers who listed a link back to their Alexa skill on their website. 

%EF: bcoz of manual curation, there is no ideal world anymore.
%In an ideal world where voice assistant ecosystems adopt our design recommendations (Section~\ref{sec:reco}), the Mapper table will be able to securely identify all skills. We simulate such a possibility and find that \sys will be able to securely predict \predIdealVal of critical user skills (Figure~\ref{fig:crit_app_correlation_ideal}). We observe that there is still a small fraction of skills that cannot be predicted --- this is because the users in our data collection effort did not have any counterpart activity for those skills. As we have discussed, users can erase their browsing history causing \sys to miss out on activity. However, in a real deployment scenario, this will be a non-issue because \sys operates continuously. 


%identifying a user's skills. Further, we perform an end-to-end evaluation of \sys by conducting skill invocation trials on a test Amazon Alexa account. To automate the skill invocation process, we use Google's Text-To-Speech (GTTS) library to generate invocation audio, and Alexa Voice Service (AVS) to automate interaction with Alexa backend. The skill invocation audio is of the form - "Alexa, open <skill invocation phrase>". We terminate our interaction with the AVS once a skill invocation occurs or if Alexa is unable to process the request. 


%In practice, we found that large swathes of the total published skill set are rife with noise from skills that lack security-critical functionality or that contain inconsequential phonetic invocations.

%\paragraph{\textbf{Analysis}}
%We utilize the collected data to run a trace-based evaluation of \sys. For each user, we have the set of preferred Alexa skills and counterpart activity(android apps and browser history domains). We look at how many of the user's critical skills can be predicted using the counterpart activity. To compute this, we first generate a set of suggested skills using only the counterpart data which involves extracting certificates from the visited websites and installed apps followed by a look-up in the mapper table. The intersection between the suggested set and the user's preferred set of skill denotes the skills that were successfully predicted by \sys.

%Then, for each user in the user study, we extract their counterpart activity as well as the list of their preferred skills. We perform skill invocation trials for each of the user's preferred skills. Firstly, we invoke all the skills without \sys and observe the invocation accuracy. Then, we configure \sys  using the counterpart data. This involves predicting skills via look-up in the mapper table and then enabling all the predicted skills while disabling all the phonetically neighbouring skills. We again invoke all the skill to test the skill invocation accuracy in presence of \sys.

%\paragraph{\textbf{Findings}}
%On average, \sys  is able to successfully predict \predVal of critical skills that a user interacts with.  A total of \totalUserSkills critical skills were collected as user preferred skills in the user study comprising of 62 unique skills. Among the 62 unique skills, 21 skills had entries in the mapper table. 
%\bigbreak
%
%\mjrev{
%MAYBE REMOVE THIS SUBSECTION
%\noindent\textbf{Invocation Correctness.} Once \sys configures the skills for users in our trace-based evaluation, we experimentally show that only the used skills execute in response to ambiguous voice commands, despite the presence of skills with phonetically close invocation phrases. Using a test Alexa account, we then feed synthesized voice\footnote{Using the Google Text-To-Speech library.} using the Alexa Voice Service to perform systematic skill invocations. We perform a total of \totalUserSkills skill invocation trials --- once for each user's skill from the data collection effort. Without \sys, we observe $105$ invocations of the correct skill and $13$ invocations of the incorrect one. For the remaining $16$ trials, Alexa could not understand the request. We then activated \sys and re-ran the same experiment for the $13$ incorrect invocations. We find a $77\%$ reduction in invocation errors (i.e., only $3$ skills were invoked incorrectly). This reduction is not $100\%$ because not all skills can be securely linked to their domains (due to unreliable vetting and absence of secure backlinks). }


\begin{figure}[t]
    \centering
    \begin{minipage}{.48\textwidth}
        \centering
        \includegraphics[width=0.98\linewidth]{images/error_rate.pdf}
        \caption{\textbf{Error Rate and Security-Usability Tradeoff: } describes the error rates (FAR and FRR) for different phonetic graph distance threshold.}
        \label{fig:error_rate}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=0.98\linewidth]{images/setup_time.pdf}
        \caption{\textbf{Initial Setup Time: } describes \sys's initial setup time for different phonetic graph distance threshold.}
        \label{fig:setup_time}
    \end{minipage}
\end{figure}

% \ifnum\flagShowFigTable=1
% \begin{figure}[t]
%     \includegraphics[width=0.5\columnwidth]{images/error_rate.pdf}
%     \caption{\textbf{Error Rate and Security-Usability Tradeoff: } describes the error rates (FAR and FRR) for different phonetic graph distance threshold. The equal error rate is achieved near the value 500.}
%     \label{fig:error_rate}
% \end{figure}
% \fi

% \ifnum\flagShowFigTable=1
% \begin{figure}[t]
%     \includegraphics[width=0.5\columnwidth]{images/setup_time.pdf}
%     \caption{\textbf{Initial Setup Time: } describes \sys's initial setup time for different phonetic graph distance threshold.}
%     \label{fig:setup_time}
% \end{figure}
% \fi

\mjrev{
\noindent\textbf{Security-Usability Tradeoff.} We evaluate \sys's performance by computing the FRR and FAR metrics, for different values of the phonetic graph distance threshold. FRR measures the usability while FAR measures the security of the system. Figure \ref{fig:error_rate} shows the FAR and FRR for different distance threshold values. Moreover, \sys's usability is also influenced by it's initial setup time. Figure \ref{fig:setup_time} shows the initial setup time as a function of the threshold value. With an increase in the distance threshold value, \sys needs to disable a larger number of skills leading to a smaller FAR, and larger values of FRR and setup time. Hence, \sys can tune the distance threshold value to achieve a desired usability-security setting. An optimal value of distance would balance and minimize all the three criterion  - FRR, FAR and initial setup time. From Figure \ref{fig:error_rate} and Figure \ref{fig:setup_time}, we see that a distance value of around 500 provides a FRR of 9.17\%, a FAR of \far, and a initial setup time of 270 minutes. Moreover, the Equal Error Rate is around 16\% and is achieved for a threshold value between 500 and 600. 
}

% EF: bcoz of manual curation, there is no ideal world anymore.
%In an ideal world where the prediction accuracy is higher because the Mapper table is complete, the number of incorrect skill invocations would be $2$ for our set of user traces --- a $77\%$ decrease in invocation errors. We again observe that his number is not a $100\%$ because even in the idealized setting of a complete Mapper table, for our user traces, there was no counterpart activity data for a small fraction of skills, thus preventing any prediction from occurring. As we have noted before, this issue goes away during a real deployment of \sys where it would have continuous access to counterpart activity.


%\ah{Need to update with latest data}
%We perform a total of \totalUserSkills skill invocation trials - 114 correct invocations, 9 incorrect invocations. For 10 trials, Alexa was not able to process the request. The 9 incorrect invocations are potential skill squatting instances.
%For the second set of invocation trials after configuring \sys , the number of incorrect invocations was reduced to 6. Among the \totalUserSkills skills that were invoked, only 54 had entries in the mapper table. For the ideal scenario where all skills have backlinks, the number of incorrect invocations was reduced to 2.



\subsection{Q4. Security and Privacy Analysis}\label{security-analysis}
% reiterate assumptions for security guarantees.
Per our threat model, the attacker is a malicious skill that tries to get executed by leveraging various design flaws in the Alexa ecosystem. The user's browser, smartphone and the legitimate skill developer's websites are trusted and not compromised. An attacker could try to compromise a legitimate website to include a fake link to their attack skill. Because of \sys however, the bar for the attack is now much higher than just uploading a malicious skill to a loosely-vetted marketplace.




% adaptive:
% 0. attacker tries to compromise legit website.
% 1. attacker injects text on website that supports user-generated content to trick backlink analysis
% 2. attacker tricks user into visiting fake website so that their counterpart activity is poisoned
% 3. attacker can try to create a phonetically-close skill JUST outside the phonetic radius threshold we set. 
% 4. privacy-respect collection of web+android history: no transmit

\subsubsection{Adaptive Attack Analysis}
We consider an adaptive attacker with knowledge of how \sys works. Concretely, this attacker can: (1) trick the user into visiting a fake website such that the counterpart activity  is poisoned; (2) inject text on a legitimate skill developer website that supports user-generated content so that the backlink analysis is tricked; (3) create a skill whose invocation phrase is just outside the phonetic radius of the legitimate skill in an attempt to still leverage voice confusion attacks. As we discuss below, our work prevents these attacks by design. 

\noindent\textbf{Counterpart activity poisoning.} An attacker can trick the user into clicking on websites they control and link those websites to a malicious skill. This can result in malicious skills getting enabled because \sys mistakenly interprets the malicious websites as the user's intention. \sys prevents this attack using its website history filtering technique discussed in Section~\ref{site_history_filter}. An attacker could also try to trick the user into installing an Android app they control. This is a harder task than just uploading a malicious skill to a loosely-vetted marketplace. The attacker has to create an Android app, get it past Google Play's strict vetting policies~\cite{alexavetting, hu2020case} and then trick the user into installing the application. Thus, \sys raises the bar for a voice confusion attack.

\noindent\textbf{Fake URL injection on legitimate website.} If a legitimate skill developer's website supports user-generated content (e.g., a help forum), an attacker can insert a URL to their attack skill, thus tricking \sys into linking the legitimate website's identity with the fake skill. Our backlink analysis prevents this attack by excluding user-generated pages.

\noindent\textbf{Phonetic threshold attack.} The malicious skill developer can choose an invocation phrase that lies just outside the phonetic cluster of an enabled skill. This can lead to a voice-based confusion attack. In Section \ref{eval_enable_disable}, we demonstrate that the probability of incorrect invocation decreases for a higher threshold. Hence, choosing a conservative threshold makes it harder to induce a voice confusion attack.

\subsubsection{Privacy Analysis}
The \sys extension accesses website history and list of installed Android apps. However, it does not store any of this information, not even on the locally. It also does not transmit it to the server, and only receives the mapper table. It just computes on this information locally using the mapper table. The only information communicated to Amazon is the set of enabled and disabled skills. The set of enabled ones can leak a small amount of information to Amazon if there are skills that user does not eventually use. Concretely, it leaks information that a website corresponding to that skill was visited. This is a small amount of information compared to existing privacy issues with systems like voice assistants~\cite{alexavetting, hu2020case, shezan-www2020} and is reasonable compared to the security advantage of preventing voice confusion attacks.

\color{black}








%\mjrev{
%\noindent\textbf{Characterizing Errors:} 
%We evaluate \sys in terms of two types of errors - (1) False Rejection Rate (FRR), and (2) False Acceptance Rate (FAR). FRR measures the probability of a used skill being rejected. For \sys, this corresponds to the probability of a used skill being disabled. FAR measures the probability where a malicious skill is missed by \sys and is not disabled. In Section x, we show that a pair of skills with a phonetic distance of more than 400 do not lead to ambiguous invocation. Using this empirical measure, we consider unused skills, with a distance of less than 400 from any used skill, to be malicious. 
%}





%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\columnwidth]{images/ndss-2021/back_link_threshold.pdf}
%    \caption{\textbf{Matched skills vs Rank threshold:} Demonstrates the number of skills with backlinks for different values of rank threshold}
%    \label{fig:back_link_threshold}
%\end{figure}

%\begin{figure*}[!t]
% \centerline{
%\subfloat[\textbf{User Study Critical Application Correlation:} %Demonstrates the ratio of enabled critical skills over the total number of critical skills present.]
%{\includegraphics[width=3.25in]{ccs-2021/images/recovered_vapps_ratio_54.pdf}%
%\label{fig:crit_app_correlation}}
%\hfill
%\subfloat[\textbf{User Study Critical Application Correlation(Ideal case):} Demonstrates the ratio of enabled critical skills over the total number of critical skills present for the ideal case when all skills pass the backlink filter]
%{\includegraphics[width=3.25in]{ccs-2021/images/recovered_vapps_ratio_ideal_54.pdf}%
%\label{fig:crit_app_correlation_ideal}}
%}
%\caption{
% User study - 
% Ratio  of  each user's critical  skills intersecting  with  the  suggested  set  over  the  total  critical  skills for different phonetic distance thresholds}
%App-Skill Correlation user study results analyzing the critical skills chosen by \sys  and all critical skills
% User Study Graphs
%}
%\label{fig:user_study}
%\end{figure*}  

%\ifnum\flagShowFigTable=1
%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.5\columnwidth]{images/recovered_vapps_ratio_ideal_57.pdf}
%    \caption{\textbf{User Study Critical Skill Prediction Rate: } demonstrates the ratio of critical skills predicted by \sys  over the total number of preferred critical skills.}
%    \label{fig:crit_app_correlation}
%\end{figure}
%\fi

%\mjrev{
%\subsubsection{Results}
%Using the data from our collection effort, we perform a trace-based evaluation of \sys to study it's effectiveness in ensuring invocation correctness for these skills despite the presence of voice confusion attacks. We also evaluate \sys's performance in terms of FAR, FRR and configuration time.}

%\mjrev{
%\noindent\textbf{Skill Enable Accuracy.} 
%For each user, we generate a list of critical mapped skills by running the extension module on the collected counterpart data. Recall that the set of critical skills are ones that are likely to be squatted upon~\cite{shezan-www2020}. This involves extracting certificates from the visited websites and installed Android apps and then indexing the Mapper table. This produces a set of suggested skills. We then look at the phonetic neighbourhood (distance threshold less than 400) of each of the user's used skills (reported in the data collection). As this phonetic neighbourhood represents skills that can cause ambiguous invocations, we use set of suggested skills to enforce the user's preference. Hence, \sys's effectiveness is represented by the percentage of used skills that can be identified among their neighbourhoods.
% Across all users ($N=$ \numUsersTotal), for a distance threshold of 500, \sys is able to correctly enable the user's preference for \coverage of critical skills that a user is likely going to interact with. Figure~\ref{fig:crit_app_correlation} shows the distribution of the enable accuracy across users. }
%A total of $69$ unique skills existed across all users (some of these were common across users making for a total of \totalUserSkills installations). Out of the $69$, our Mapper table had entries for $21$. This represents the number of skill developers who listed a link back to their Alexa skill on their website. 

%EF: bcoz of manual curation, there is no ideal world anymore.
%In an ideal world where voice assistant ecosystems adopt our design recommendations (Section~\ref{sec:reco}), the Mapper table will be able to securely identify all skills. We simulate such a possibility and find that \sys will be able to securely predict \predIdealVal of critical user skills (Figure~\ref{fig:crit_app_correlation_ideal}). We observe that there is still a small fraction of skills that cannot be predicted --- this is because the users in our data collection effort did not have any counterpart activity for those skills. As we have discussed, users can erase their browsing history causing \sys to miss out on activity. However, in a real deployment scenario, this will be a non-issue because \sys operates continuously. 


%identifying a user's skills. Further, we perform an end-to-end evaluation of \sys by conducting skill invocation trials on a test Amazon Alexa account. To automate the skill invocation process, we use Google's Text-To-Speech (GTTS) library to generate invocation audio, and Alexa Voice Service (AVS) to automate interaction with Alexa backend. The skill invocation audio is of the form - "Alexa, open <skill invocation phrase>". We terminate our interaction with the AVS once a skill invocation occurs or if Alexa is unable to process the request. 


%In practice, we found that large swathes of the total published skill set are rife with noise from skills that lack security-critical functionality or that contain inconsequential phonetic invocations.

%\paragraph{\textbf{Analysis}}
%We utilize the collected data to run a trace-based evaluation of \sys. For each user, we have the set of preferred Alexa skills and counterpart activity(android apps and browser history domains). We look at how many of the user's critical skills can be predicted using the counterpart activity. To compute this, we first generate a set of suggested skills using only the counterpart data which involves extracting certificates from the visited websites and installed apps followed by a look-up in the mapper table. The intersection between the suggested set and the user's preferred set of skill denotes the skills that were successfully predicted by \sys.

%Then, for each user in the user study, we extract their counterpart activity as well as the list of their preferred skills. We perform skill invocation trials for each of the user's preferred skills. Firstly, we invoke all the skills without \sys and observe the invocation accuracy. Then, we configure \sys  using the counterpart data. This involves predicting skills via look-up in the mapper table and then enabling all the predicted skills while disabling all the phonetically neighbouring skills. We again invoke all the skill to test the skill invocation accuracy in presence of \sys.

%\paragraph{\textbf{Findings}}
%On average, \sys  is able to successfully predict \predVal of critical skills that a user interacts with.  A total of \totalUserSkills critical skills were collected as user preferred skills in the user study comprising of 62 unique skills. Among the 62 unique skills, 21 skills had entries in the mapper table. 
%\bigbreak
%
%\mjrev{
%MAYBE REMOVE THIS SUBSECTION
%\noindent\textbf{Invocation Correctness.} Once \sys configures the skills for users in our trace-based evaluation, we experimentally show that only the used skills execute in response to ambiguous voice commands, despite the presence of skills with phonetically close invocation phrases. Using a test Alexa account, we then feed synthesized voice\footnote{Using the Google Text-To-Speech library.} using the Alexa Voice Service to perform systematic skill invocations. We perform a total of \totalUserSkills skill invocation trials --- once for each user's skill from the data collection effort. Without \sys, we observe $105$ invocations of the correct skill and $13$ invocations of the incorrect one. For the remaining $16$ trials, Alexa could not understand the request. We then activated \sys and re-ran the same experiment for the $13$ incorrect invocations. We find a $77\%$ reduction in invocation errors (i.e., only $3$ skills were invoked incorrectly). This reduction is not $100\%$ because not all skills can be securely linked to their domains (due to unreliable vetting and absence of secure backlinks). }

% \ifnum\flagShowFigTable=1
% \begin{figure}[t]
%     \includegraphics[width=0.5\columnwidth]{images/error_rate.pdf}
%     \caption{\textbf{Error Rate and Security-Usability Tradeoff: } describes the error rates (FAR and FRR) for different phonetic graph distance threshold. The equal error rate is achieved near the value 500.}
%     \label{fig:error_rate}
% \end{figure}
% \fi

% \ifnum\flagShowFigTable=1
% \begin{figure}[t]
%     \includegraphics[width=0.5\columnwidth]{images/setup_time.pdf}
%     \caption{\textbf{Initial Setup Time: } describes \sys's initial setup time for different phonetic graph distance threshold.}
%     \label{fig:setup_time}
% \end{figure}
% \fi

%\mjrev{
%\noindent\textbf{Security-Usability Tradeoff.} We evaluate \sys's performance by computing the FRR and FAR metrics, for different values of the phonetic graph distance threshold. FRR measures the usability while FAR measures the security of the system. Figure \ref{fig:error_rate} shows the FAR and FRR for different distance threshold values. Moreover, \sys's usability is also influenced by it's initial setup time. Figure \ref{fig:setup_time} shows the initial setup time as a function of the threshold value. With an increase in the distance threshold value, \sys needs to disable a larger number of skills leading to a smaller FAR, and larger values of FRR and setup time. Hence, \sys can tune the distance threshold value to achieve a desired usability-security setting. An optimal value of distance would balance and minimize all the three criterion  - FRR, FAR and initial setup time. From Figure \ref{fig:error_rate} and Figure \ref{fig:setup_time}, we see that a distance value of around 500 provides a FRR of 9.17\%, a FAR of \far, and a initial setup time of 270 minutes. Moreover, the Equal Error Rate is around 16\% and is achieved for a threshold value between 500 and 600. 
%}

% EF: bcoz of manual curation, there is no ideal world anymore.
%In an ideal world where the prediction accuracy is higher because the Mapper table is complete, the number of incorrect skill invocations would be $2$ for our set of user traces --- a $77\%$ decrease in invocation errors. We again observe that his number is not a $100\%$ because even in the idealized setting of a complete Mapper table, for our user traces, there was no counterpart activity data for a small fraction of skills, thus preventing any prediction from occurring. As we have noted before, this issue goes away during a real deployment of \sys where it would have continuous access to counterpart activity.


%\ah{Need to update with latest data}
%We perform a total of \totalUserSkills skill invocation trials - 114 correct invocations, 9 incorrect invocations. For 10 trials, Alexa was not able to process the request. The 9 incorrect invocations are potential skill squatting instances.
%For the second set of invocation trials after configuring \sys , the number of incorrect invocations was reduced to 6. Among the \totalUserSkills skills that were invoked, only 54 had entries in the mapper table. For the ideal scenario where all skills have backlinks, the number of incorrect invocations was reduced to 2.


==> z_related_work.tex <==
\section{Related Work}

% attacks on voice assistants
\noindent\textbf{Voice-based confusion attacks.} Kumar et al. introduced skill squatting attacks, where a malicious developer registers a phonetically similar sounding skill as the target~\cite{kumar}. Zhang N. et al. perform a similar analysis for Google Home, and introduce an additional attack where a fake skill masquerades as a true one~\cite{zhang}. Finally, Zhang Y. et al. introduce \textit{lapsus} attacks that rely on common speech variation among humans~\cite{lipfuzzer}. For example, given a \appv with invocation \textit{``the true bank skill,''} a user might misspeak and instead ask for \textit{``the truth bank skill.''} 
%An attacker can systematically discover common speech variations for a given phrase and then register skills. 
Broadly, all these attacks define a class of voice-based confusion attacks. The fundamental cause is the mismatch between a user's intention and the voice assistant's behavior.
%Our goal is to anticipate a user's intentions by analyzing contextual information from their counterpart apps and then enforce those intentions using a secure system design.

\noindent\textbf{Design Issues in Alexa Ecosystem.} Lentzsch et al. recently performed a security analysis of the Alexa ecosystem that includes the vetting processes~\cite{alexa-skill-ecosystem-2021}. Like us, they find that attackers can circumvent the vetting and upload malicious skills to launch voice confusion attacks. They also observe that an attacker can mirror the metadata of legitimate skills, lending further confirmation that the ecosystem currently lacks any notion of secure identity. By contrast, our work contributes a method to provide a secure identity to skills through backlink search. 

% defenses aginst voice-based confusion attacks
\noindent\textbf{Existing Defenses.} A direct way to combat voice-based confusion attacks is to prevent \appvs from being created with overlapping or identically-sounding invocation phrases. Kumar et al. suggest a phoneme-based analysis to detect similar-sounding skills ~\cite{kumar}. Amazon Alexa includes developer guidelines that explicitly prohibit duplicate names~\cite{alexa-guidelines}. However, these guidelines are not technically enforced. Recent changes to Alexa indicate that they now perform manual vetting, which is not scalable. Google Home's manual analysis detects when an invocation phrase is too close to an existing one. Although this seems like a reasonable approach, there are pitfalls. For instance, Google Home is prone to a phenomenon similar to domain squatting --- a third-party developer scoops up invocation phrases that heavily overlap existing and popular services (e.g., Lyft, Papa John's), preventing the first parties from creating \appvs with those invocation phrases~\cite{voicebot}. This also has the effect of third-parties benefiting from the copyright and reputation of the first-party invocation phrases on which they squat. %Furthermore, the lapsus attacks discussed above do not require the attacker to mirror the target invocation phrases completely. 
In summary, although these techniques add defense-in-depth, they do not address the root cause of the problem.

Zhang N. et al. suggest a skill response checker that keeps track of the current skill's responses and computes a similarity score to other skills~\cite{zhang}. If two skills are found to be similar enough, an alarm is generated. Our work is orthogonal and represents a systems-oriented defense that securely predicts and enables skills using counterpart app information. We observe that a secure voice assistant platform benefits from both approaches.

Guo et al. built SkillExplorer, an NLP-based testing system that uncovers potentially policy-violating behavior~\cite{skillex}. By contrast, our work ensures that only the user-intended skills run in response to ambiguous utterances and does not pass judgment on whether the authorized skill violates policies. 




%\noindent\textbf{Physical attacks on voice assistants.} A large body of recent work attacks voice assistants physically by injecting commands that exploit the ML models using adversarial examples~\cite{hvc,noodles,devil} or the non-linear components of microphones~\cite{dolphin,commander-song,inaudble} or the photoacoustic effect~\cite{sugawara2020light}. From the perspective of our defense, these are simply voice commands that come from a non-human source. Our work is independent of the origin of a command. It focuses on ensuring that the voice assistant only executes legitimate skills that match the counterpart apps of a user. 
\noindent\textbf{Attacks on Speech Processing.} A large body of recent work attacks voice assistants physically by injecting commands that exploit the ML models using adversarial examples~\cite{hvc,noodles,devil} or the non-linear components of microphones~\cite{dolphin,commander-song,inaudble} or the photoacoustic effect~\cite{sugawara2020light}. From \sys\xspace's perspective, these are simply voice commands that come from a non-human source. Our work is independent of the origin of a command, and it is not intended to address physical attacks. Instead, this work focuses on ensuring the voice assistant only executes legitimate skills that match the counterpart activity of a user. 

%\noindent\textbf{IoT Security.} Current research focuses on the systems security issues of appified platforms~\cite{smartthings16,ifttt16,contexiot17}, and the IoT devices~\cite{smartlocks,iot-nuclear}. Ho et al. discovered security problems in smart locks~\cite{smartlocks}, and Ronen et al. showed how worms could propagate among vulnerable devices~\cite{iot-nuclear}. Fernandes et al. found a series of design issues in the SmartThings IoT platform~\cite{smartthings16}. Systems like FlowFence~\cite{flowfence16}, ContexIoT~\cite{contexiot17}, and SmartAuth~\cite{smartauth} use data flow or context extraction techniques to mitigate the security issues. %By contrast, our work, to the best of our knowledge, is the first systems-oriented approach to defending voice assistant platforms against squatting attacks.


